From Paradigm Shift to Audit Rift: Empirical Analysis and Validation of Security Audit Methodologies for Asynchronous Smart Contract Systems

The Open Network (TON) is a high-performance blockchain platform designed for scalability and efficiency, leveraging an asynchronous execution model and a multi-layered architecture. While TON's design offers significant advantages, it also introduces unique challenges for smart contract development and security. This paper introduces a comprehensive audit checklist for TON smart contracts, based on an empirical analysis of 34 professional audit reports containing 233 real-world vulnerabilities. The checklist addresses TON-specific challenges, such as asynchronous message handling, and provides actionable insights for developers and auditors. We also present detailed case studies of vulnerabilities in TON smart contracts, highlighting their implications and offering lessons learned. To validate practical utility, we conducted a practitioner survey (n=11 complete responses), confirming the checklist's value alongside automated tools. By adopting this checklist, developers and auditors can systematically identify and mitigate vulnerabilities, enhancing the security and reliability of TON-based projects. Our work bridges the gap between Ethereum's mature audit methodologies and the emerging needs of the TON ecosystem, fostering a more secure and robust blockchain environment.

==> misc.tex <==
% \section*{Funding}

% \section*{Acknowledgments}

% \section{\todo{Related Work}}
% \label{section:RelatedWork}

% Smart Contract Vulnerabilities in Other Blockchains
% \begin{itemize}
%     \item 
%         Review common vulnerabilities in platforms like Ethereum (e.g., reentrancy, overflow).
%     \item 
%         Discuss existing security analyses and auditing tools.
% \end{itemize}

% Previous Studies on TON Smart Contracts
% \begin{itemize}
%     \item 
%         Identify any prior research focused on TON security.
%     \item 
%         Discuss studies on asynchronous execution and its challenges.
% \end{itemize}

% Audit Practices and Methodologies
% \begin{itemize}
%     \item 
%         Summarize standard audit procedures for smart contracts.
%     \item 
%         Highlight tools and frameworks used in auditing.
% \end{itemize}

% Research Gap: 
% Emphasize the need for TON-specific security analysis and audit guidelines.

% \section{\todo{Background: TON Virtual Machine and Asynchronous Transaction Execution}}
% \label{section:Background}

% Overview of The Open Network (TON)
% \begin{itemize}
%     \item 
%         Introduce TON as a blockchain platform.
%     \item 
%         Describe its architecture and consensus mechanism.
% \end{itemize}

% TON Virtual Machine (TVM)
% \begin{itemize}
%     \item 
%         Explain the role of TVM in executing smart contracts.
%     \item 
%         Discuss the programming languages supported (e.g., FunC).
% \end{itemize}

% Asynchronous Transaction Execution
% \begin{itemize}
%     \item 
%         Define asynchronous execution in the context of TON.
%     \item 
%         Illustrate how messages and smart contracts interact asynchronously.
%     \item 
%         Compare synchronous vs. asynchronous execution models.
% \end{itemize}

% Implications for Smart Contract Development
% \begin{itemize}
%     \item 
%         Highlight the benefits of asynchronous execution (e.g., scalability).
%     \item 
%         Discuss the potential security risks introduced.
% \end{itemize}

% \section{Checklist for Auditing TON Smart Contracts}

% In this section, we introduce our checklist, which is publicly available on GitHub \cite{TODO}. The checklist is based on publicly available audit reports and our internal auditing practices. It serves as a heuristic tool rather than a theoretically justifiable or inducible framework. The checklist provides a structured approach to auditing TON smart contracts, emphasizing the minimization of false negatives (Type II errors) while allowing for some tolerance of false positives (Type I errors) and redundant efforts. It is organized sequentially, guiding auditors from a general understanding of the contract to deeper analysis of vulnerabilities and best practices.

% The checklist is divided into the following sections: Contract Design, Asynchronous Execution, Common Vulnerabilities, Gas Control, Random Number Generation, Language-Specific Errors (FunC and Tact), Best Practices. Let us go through it with key details.

% \subsection{Contract Design}
% Begin by mapping all message flows to understand how messages are processed and routed. Identify all entry points and analyze how input data and incoming messages are handled, including error handling. Ensure that the contract has robust authorization checks for all functions and message handlers. Evaluate the contract structure for unnecessary centralization and consider how the contract handles partial execution of transactions, especially in cases of gas exhaustion.

% \subsection{Asynchronous Execution}
% TON's asynchronous execution model introduces unique challenges. Messages are guaranteed to be delivered but not in a predictable timeframe, and their order is only predictable if sent to the same contract (using \textbf{logical time}). Consider the impact of concurrent processes and how state changes might occur between message flows. Analyze external dependencies and ensure that operations are independent of the sequence of message arrivals.

% \subsection{Common Vulnerabilities}
% Address the public nature of blockchain data, ensuring that sensitive information like passwords or keys is never transmitted. Properly handle bounced messages to avoid issues such as tokens being sent to the void. Guard against unrestricted data recording, logical errors, and replay attacks by using mechanisms like \textbf{seqno}. Implement the \textbf{carry-value pattern} for inter-contract value transfers and ensure storage compatibility during smart contract updates. Avoid mixing signed and unsigned numbers in calculations and use exit codes correctly, avoiding reserved values. Prevent denial-of-service attacks by avoiding infinite or excessively long loops and ensure proper parsing and serialization of data.

% \subsection{Gas Control}
% Carefully calculate gas costs to ensure sufficient gas for operations and implement logic to return excess gas to the sender. Avoid data structures that can grow infinitely, as they increase gas costs over time. Recognize the risks of partial fulfillment when running out of gas and optimize storage parsing efficiency to minimize gas consumption.

% \subsection{Random Number Generation}
% Be cautious with randomness generation, as validators can influence the outcome. In Tact, use \textbf{nativeRandom} or \textbf{nativeRandomInterval} instead of \textbf{randomInt} and \textbf{random} to ensure secure randomness.

% \subsection{Language-Specific Errors}
% In FunC, use the \textbf{impure} modifier correctly for state-changing functions and carefully manage storage, variable ordering, and variable overrides. In Tact, avoid modifying parameters of incoming messages or functions and exercise caution when using assembler and native functions.

% \subsection{Best Practices}
% Replace magic numbers with named constants for clarity and maintain thorough documentation of the contract's functionality and design decisions. Conduct independent code reviews and ensure the contract adheres to relevant TON standards and best practices.

% \subsection{Checklist in Numbers}

% By following this checklist, auditors can systematically assess the security and robustness of TON smart contracts, identifying potential vulnerabilities and ensuring reliable operation within the TON ecosystem. Here are numerical details about the considered reports based on audit reports.

% \begin{figure}[htbp]
% \centering
% \begin{forest}
% for tree={
%   grow'=0,
%   child anchor=west,
%   parent anchor=east,
%   anchor=west,
%   calign=first,
%   edge path={
%     \noexpand\path[\forestoption{edge}]
%     (!u.south west) +(5pt,0) |- (.child anchor)\forestoption{edge label};
%   },
%   before typesetting nodes={
%     if n=1
%       {insert before={[,phantom]}}
%       {}
%   },
%   fit=band,
%   before computing xy={l=12pt},
%   s sep=2pt,
%   l sep=8pt,
% }
% [Vulnerabilities 233
%   [Asynchronous Execution 6
%     [Key Considerations 6]
%   ]
%   [Best Practices 36
%     [Code Review 7]
%     [Compliance with Standards 5]
%     [Documentation 23]
%     [Magic Numbers-Flags-and Constants 1]
%   ]
%   [Common Errors 92
%     [Bounced Message Handlers 3]
%     [Carry-Value Pattern 1]
%     [Exit Codes 2]
%     [Logical Errors 70]
%     [Parsing and Serialization 6]
%     [Public Nature of Blockchain 2]
%     [Replay Attack 3]
%     [Restrictions on Data Recording 1]
%     [Sending Messages from Loops 1]
%     [Smart Contract Update 2]
%     [Smart Contract Updates 1]
%   ]
%   [Contract Design 76
%     [Authorization Checks 25]
%     [Contract Design and Centralization 19]
%     [External Message Handling 1]
%     [Input Data Processing 15]
%     [Logical Errors 8]
%     [Message Generation and Handling 2]
%     [Partial Execution of Transactions 6]
%   ]
%   [Gas Control 18
%     [Moderate Handling of Gas 18]
%   ]
%   [Possible Errors in FunC 4
%     [Function Modifiers 1]
%     [Modifying Variables 2]
%     [Storage Management 1]
%   ]
%   [Random Number Generation in TON 1
%     [Safe Randomness Generation 1]
%   ]
% ]
% \end{forest}
% \caption{The number of vulnerabilities in TON smart contracts audits per checklist category.}
% \label{fig:vulnerabilities_tree}
% \end{figure}






\section{\todo{Asynchronous Execution Vulnerabilities}}

Understanding Asynchronous Vulnerabilities
\begin{itemize}
    \item Explain how asynchronous execution differs from synchronous models.
    \item Discuss why traditional security measures may not suffice.
\end{itemize}

Types of Asynchronous Vulnerabilities
\begin{itemize}
    \item \textbf{Reentrancy Issues}
    \begin{itemize}
        \item Describe how reentrancy can occur in asynchronous contexts.
        \item Provide examples relevant to TON.
    \end{itemize}
    \item \textbf{State Inconsistency}
    \begin{itemize}
        \item Explain how delayed state updates can lead to vulnerabilities.
    \end{itemize}
    \item \textbf{Message Ordering and Timing Attacks}
    \begin{itemize}
        \item Discuss risks associated with unpredictable message processing order.
    \end{itemize}
\end{itemize}

Practical Demonstrations
\begin{itemize}
    \item \textbf{Code Examples}
    \begin{itemize}
        \item Present code snippets illustrating vulnerable smart contracts.
        \item Annotate code to highlight the vulnerability points.
    \end{itemize}
    \item \textbf{Execution Schemas (Diagrams)}
    \begin{itemize}
        \item Provide visual diagrams showing the flow of asynchronous calls.
        \item Illustrate how an attacker could exploit the vulnerabilities.
    \end{itemize}
\end{itemize}

Exploitation Scenarios
\begin{itemize}
    \item \textbf{Attack Vectors}
    \begin{itemize}
        \item Describe possible strategies an attacker might use.
    \end{itemize}
    \item \textbf{Potential Impact}
    \begin{itemize}
        \item Discuss the consequences of successful exploitation (e.g., funds theft).
    \end{itemize}
\end{itemize}

Mitigation Techniques
\begin{itemize}
    \item Offer best practices for developers to avoid these vulnerabilities.
    \item Suggest coding patterns and security checks specific to asynchronous execution.
\end{itemize}

\section{Systematization of Vulnerabilities}

Framework Development
\begin{itemize}
    \item Propose a systematic approach to categorize and address vulnerabilities.
    \item Align the framework with the unique aspects of TON's architecture.
\end{itemize}

Mapping Vulnerabilities to Risks
\begin{itemize}
    \item Connect identified vulnerabilities with potential risks and impacts.
\end{itemize}

Audit Checklist Creation
\begin{itemize}
    \item \textbf{Structure of the Checklist}
    \begin{itemize}
        \item Organize the checklist into sections (e.g., contract design, state management).
        \item Include general security considerations and TON-specific items.
    \end{itemize}
    \item \textbf{Detailed Checklist Items}
    \begin{itemize}
        \item List actionable audit points with explanations.
        \item Emphasize checks for asynchronous execution issues.
        \item Provide examples or references where applicable.
    \end{itemize}
\end{itemize}

\section{\todo{Conclusions}}

**TODO** May be useful

Key findings include the identification of vulnerabilities unique to TON's asynchronous nature, such as delayed state updates and race conditions. While current audit practices effectively identify traditional vulnerabilities, specialized tools and methodologies tailored to TON's architecture are needed to address its unique challenges and ensure comprehensive security coverage.

**ENDTODO**

Summary of Findings
\begin{itemize}
    \item Recap the key vulnerabilities identified in TON smart contracts.
    \item Highlight the significance of asynchronous execution in introducing security risks.
\end{itemize}

Contributions Revisited
\begin{itemize}
    \item Reiterate the development of the audit checklist and its importance.
    \item Emphasize the practical demonstrations provided.
\end{itemize}

Implications for the TON Ecosystem
\begin{itemize}
    \item Discuss how the findings can improve smart contract security.
    \item Encourage the adoption of the checklist by developers and auditors.
\end{itemize}

Future Work
\begin{itemize}
    \item Suggest areas for further research, such as automated detection tools.
    \item Propose extending the study to cover more complex contract interactions.
\end{itemize}

Closing Remarks
\begin{itemize}
    \item Reflect on the necessity of proactive security measures.
    \item Encourage collaboration within the community to enhance security practices.
\end{itemize}


